Evaluating simulation techniques for lubricant distribution in gearboxes

Efficient lubrication is crucial for the performance and durability of high-speed gearboxes, particularly under varying load conditions. Excess lubrication leads to increased churning losses, while insufficient lubrication accelerates wear on contact surfaces. Due to the high rotational speeds involved, direct experimental visualization of lubricant distribution within gearboxes is challenging, making numerical simulations indispensable. Although various modelling approaches exist, a direct comparison that jointly evaluates accuracy and computational efficiency is missing. Furthermore, studies on the computational modelling of highly viscous lubricants such as grease in gearboxes are limited. This study addresses these gaps by comparing two mesh-based Eulerian solvers (OpenFOAM and Ansys-Fluent) and two Lagrangian particle-based solvers (PreonLab and MESHFREE) for oil distribution in gearboxes. Two benchmark cases are considered: one for qualitative assessment and another for quantitative evaluation. OpenFOAM and Ansys-Fluent show good agreement with the experiment data in selected cases, but incur a significant computational cost. PreonLab performs well qualitatively, yet exhibits greater deviation in quantitative predictions. These comparisons provide information for selecting the suitable solver according to specific simulation requirements. Furthermore, the study extends to grease distribution by first validating the solver and then investigating the influence of filling volume and gear speed on the amount of grease deposited on gears. The benchmark cases presented provide a reference framework for evaluating additional solvers in future gearbox lubrication studies.

==> Sections/results_CouetteFlow.tex <==
\section{Taylor-Couette flow}

For direct comparison of the numerical methodologies with respect to accuracy and performance, they are first measured against the analytical solution of single phase circular Taylor-Couette flow [1].
\label{sec:resultscouette}
\subsection{Test case setup}

The circular Taylor-Couette flow configuration consists of a hollow cylinder with inner and outer ring covered by an upper and lower slip boundary to mimic a quasi 2D case. The inner ring, with a radius of 0.35 m, is positioned concentrically within the outer ring, which has a radius of 0.5 m. The inner ring rotates at a speed of 0.19 revolution per minute (RPM), while the outer ring remains stationary. Air is chosen as the operating fluid with a (\textcolor{red}{Check dynamic or kinematic})dynamic viscosity of \SI{10}{\micro\pascal\s} and density of 1 \si{\kilogram/\cubic\meter}.


\subsection{Results and discussion}

To evaluate the resolution dependence of each solver, a transient flow simulation is conducted. The simulations are run for 2000 seconds of real time, beyond which only minor variations in flow parameters are observed. Following the completion of the transient phase, a direct comparison of the performance and accuracy of all the methods is carried out. 
%All the setups including the result as csv* file and python scripts are made public via \textcolor{red}{Add Bosch Link}. \\

%OpenFOAM
\textit{OpenFOAM}

The influence of mesh resolution on the velocity distribution from the rotating to the stationary ring is shown in Fig. \ref{fig:Taylor_Couette_OpenFOAM_MeshStudy}. Initially, three different mesh types---hexahedral, tetrahedral, and polyhedral---are tested. To maintain uniformity, the number of cells between rotating and stationary ring are kept constant for all the mesh types. The various mesh configurations utilized in the simulation, along with the mesh employed for the mesh dependence study, are presented in Fig. \ref{fig:TaylorCouetteFlow_OF_MeshPicture}. All the cases are simulated using 4 CPUs. In all the cases, the error margin compared to the analytical values remained below 2\%. Although the total cell count for both hexahedral and polyhedral mesh is comparable, the computational time taken for the polyhedral mesh is longer. This could be due to the higher number of neighboring cells in polyhedral mesh compared to that in hexahedral mesh. Hence, the hexahedral mesh is used for mesh dependence study. The results of the mesh refinement study (Fig. \ref{fig:Taylor_CouetteFlow_MeshStudy}) show good agreement with the analytical value across all the resolutions. The mesh resolution with 8 cells exhibits the highest deviation, approximately 3\%, followed by the 27-cell configuration, while the 36-cell mesh demonstrates the lowest deviation. However, despite the lower deviation of the 36-cell mesh, its computation time is three times longer than that of the 27-cell configuration, see Fig. \ref{fig:OF_TaylorCouetteFlow_PlotForTimeTaken_MeshStudy}. Additionally, the average deviation between the 27-cell and 36-cell meshes is minimal. Therefore, it is concluded that a 27-cell resolution  provides the optimal balance of accuracy and efficiency and is selected for further study.
   
      
\begin{figure}[htbp!]
    \centering
    \begin{subfigure}{0.49\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/OpenFOAM/OF_VelocityProfile_DifferentMeshTypes.png}
        \caption{Comparison of velocity error for different mesh types against analytical solutions.}
        \label{fig:OF_Taylor_CouetteFlow_MeshTypesComparison}
    \end{subfigure} \hspace{1.2em}
    \begin{subfigure}{0.46\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/OpenFOAM/TaylorCouetteFlow_DifferentStepsForConvergence.png}
        \caption{}
        \label{fig:OF_Taylor_CouetteFlow_MeshType_TimeTaken}
    \end{subfigure}  
    \caption{Results of mesh study for transient Taylor-Couette flow simulation using OpenFOAM.}
    \label{fig:OF_Taylor_Couette_Type}
\end{figure}

\begin{figure}[htbp!]
	\centering
	\begin{subfigure}{0.49\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/OpenFOAM/OF_VelocityProfile_MeshStudy.png}
		\caption{Convergence analysis and computational time comparison across different mesh types.}
		\label{fig:Taylor_CouetteFlow_MeshSizeComparison}
	\end{subfigure} \hspace{1.2em}
	\begin{subfigure}{0.46\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/OpenFOAM/TaylorCouetteFlow_OF_MeshStudy.png}
		\caption{Comparison of velocity distribution across different mesh sizes. }
		\label{fig:OF_TaylorCouetteFlow_MeshStudy_TimeTaken}
	\end{subfigure}  
	\caption{Results of mesh study for steady-state Taylor-Couette flow simulation using OpenFOAM.}
	\label{fig:OF_Taylor_Couette_MeshStudy}
\end{figure}

\begin{figure}[htbp!]
	\centering
	\includegraphics[width=0.8\textwidth]{Figures/OF_TaylorCouetteFlow_DifferentMeshSize_MeshPicture.png}
	\caption{Result of mesh study for steady-state Taylor-Couette flow simulation using Ansys-Fluent.}
	\label{fig:TaylorCouetteFlow_OF_MeshPicture}
\end{figure}

%Ansys
\textit{Ansys - Fluent}

A mesh dependence study, similar to that conducted with OpenFOAM, is performed using Ansys-Fluent. The Fluent mesher is used to create three polyhedral-type meshes with 9, 27, and 36 cells between the rotating and stationary ring. Only polyhedral meshes are reviewed here due to the suggestion in the solver manual. For all mesh resolutions, the error remains low, with a maximum error of 3.8\%. The highest average deviation, observed with the coarse mesh (9 cells). is 0.44\%. Furthermore, the largest error is found for the same coarse mesh at the outer stationary wall, where the deviation reached 3.8\%. Similar to the findings from the OpenFOAM mesh study, the difference in deviation betweeen the two resolution, 27-cell and 36-cell is negligible. Therefore, the mesh resolution with 27 cells is selected for further studies and comparisons.      
\\
\begin{figure}[htbp!]
	\centering
	\begin{subfigure}{0.30\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/Ansys/AF_TaylorCouetteFlow_CoarseMesh.png}
		\caption{Convergence analysis and computational time comparison across different mesh types.}
		\label{fig:AF_Taylor_CouetteFlow_MeshStudy_Deviation}
	\end{subfigure} \hspace{1.2em}
    \begin{subfigure}{0.30\textwidth}
    	\centering
    	\includegraphics[width=\textwidth]{Figures/Ansys/AF_TaylorCouetteFlow_FineMesh.png}
    	\caption{Convergence analysis and computational time comparison across different mesh types.}
    	\label{fig:AF_Taylor_CouetteFlow_MeshStudy_Deviation}
    \end{subfigure} \hspace{1.2em}
    \begin{subfigure}{0.30\textwidth}
    	\centering
    	\includegraphics[width=\textwidth]{Figures/Ansys/AF_TaylorCouetteFlow_FinerMesh.png}
    	\caption{Convergence analysis and computational time comparison across different mesh types.}
    	\label{fig:AF_Taylor_CouetteFlow_MeshStudy_Deviation}
    \end{subfigure} \hspace{1.2em}
    \\
	\begin{subfigure}{0.49\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/Ansys/AF_TaylorCouetteFlow_MeshStudy.jpg}
		\caption{Convergence analysis and computational time comparison across different mesh types.}
		\label{fig:AF_Taylor_CouetteFlow_MeshStudy_Deviation}
	\end{subfigure} \hspace{1.2em}
	\begin{subfigure}{0.46\textwidth}
		\centering
		\includegraphics[width=\textwidth]{Figures/Ansys/TaylorCouetteFlow_Ansys_MeshStudy.png}
		\caption{Comparison of velocity distribution across different mesh sizes. }
		\label{fig:AF_Taylor_CouetteFlow_MeshStudy_TimeTaken}
	\end{subfigure}  
	\caption{Results of mesh study for steady-state Taylor-Couette flow simulation using OpenFOAM.}
	\label{fig:AF_Taylor_Couette_MeshStudy}
\end{figure}

%MESHFREE
\textit{MESHFREE}

MESHFREE provides two particle based approaches for modeling the particle movement: Eulerian and Lagrangian, as discussed in Sec. \ref{sec:Meshfree_Theory}. The Lagrangian method is preferred for transient simulations hence a particle study is conducted using this approach with three resolutions: 9, 27, and 36 particles between the rotating and stationary ring. With a coarse resolution of 9 particles between the rings, the velocity profile deviates from the analytical results (Fig \ref{fig:MF_TaylorCouetteFlow_MeshStudy}). In contrast, the velocity profiles for the other two resolutions, 27 and 36 particles, match well with the analytical result.  Additionally, the resolution with 27 particles produces accurate results in a shorter computation time compared to 36 particles. Therefore, it is concluded that the Lagrangian approach with 27 particles between the two rings provides the optimal balance between accuracy and computational efficiency, and this configuration is used for further comparisons.
\begin{figure}[htbp!]
    \centering
     \begin{subfigure}{0.30\textwidth}
    	\centering
    	\includegraphics[width=\textwidth]{Figures/MESHFREE/MF_TaylorCouetteFlow_Coarse.png}
    	\caption{Comparison of velocity distribution for different particle sizes using Lagrangian method.}
    	\label{fig:MF_TaylorCouetteFlow_MeshStudy_Deviation}
    \end{subfigure} \hspace{1.2em}
     \begin{subfigure}{0.30\textwidth}
    	\centering
    	\includegraphics[width=\textwidth]{Figures/MESHFREE/MF_TaylorCouetteFlow_Fine.png}
    	\caption{Comparison of velocity distribution for different particle sizes using Lagrangian method.}
    	\label{fig:MF_TaylorCouetteFlow_MeshStudy_Deviation}
    \end{subfigure} \hspace{1.2em}
     \begin{subfigure}{0.30\textwidth}
    	\centering
    	\includegraphics[width=\textwidth]{Figures/MESHFREE/MF_TaylorCouetteFlow_Finer.png}
    	\caption{Comparison of velocity distribution for different particle sizes using Lagrangian method.}
    	\label{fig:MF_TaylorCouetteFlow_MeshStudy_Deviation}
    \end{subfigure} \hspace{1.2em}
    \\
    \begin{subfigure}{0.48\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/MESHFREE/TaylorCouetteFlow_MeshfreeParticleStudy.png}
        \caption{Comparison of velocity distribution for different particle sizes using Lagrangian method.}
        \label{fig:MF_TaylorCouetteFlow_MeshStudy_Deviation}
    \end{subfigure} \hspace{1.2em}
    \begin{subfigure}{0.47\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/MESHFREE/TaylorCouetteFlow_MF_MeshStudy.png}
        \caption{Comparison of velocity distribution between Lagrangian and Eulerian approach. }
        \label{fig:MF_Taylor_CouetteFlow_ParticleStudy_TimeTaken}
    \end{subfigure}
    \caption{Results for Taylor-Couette flow using MESHFREE.}
    \label{fig:MF_TaylorCouetteFlow_MESHFREEResults}
\end{figure}


%Comparison
\textit{Comparison of different methods}

In the following, different solvers and mesh rotation methods are compared to evaluate their performance in simulating transient Taylor-Couette flow:
\begin{itemize}
	\item OpenFOAM with Rotating Wall Boundary Condition
	\item OpenFOAM with Arbitrary Mesh Interface (AMI) 
	\item Ansys-Fluent with Rotating Wall Boundary Condition
	\item Ansys-Fluent with Sliding Mesh Approach
	\item MESHFREE with Lagrangian Approach
\end{itemize}
The simulations using the Rotating Wall boundary condition in both OpenFOAM and Ansys-Fluent show minimal deviation, with OpenFOAM results slightly better than Ansys-Fluent. However, when considering the average overall deviation, OpenFOAM using the Arbitrary Mesh Interface (AMI) method exhibits the highest discrepency, followed by MESHFREE approach. Despite the lower average deviation observed in MESHFREE compared to OpenFOAM with the AMI method, MESHFREE method results in the highest error at the wall boundaries. 

In addition to having the lowest error, the simulation with the rotating wall boundary condition proves to be the most computationally efficient compared to other methods. OpenFOAM shows a clear advantage by completing the simulation in only 1 hour for 2000 seconds of real time, while Ansys-Fluent requires 23 hours for the same case. This is due to the different Pressure-Velocity coupling schemes used. OpenFOAM, using the pimpleFoam solver, implements the pimple loop -- a combination of PISO and simple. In contrast, Ansys-Fluent recommends the simple loop for transient simulations. Furthermore, the simulation time for methods using sliding mesh and AMI is three times longer than that of the rotating wall condition. The simulation time of MESHFREE method falls between that of the rotating wall and sliding mesh or AMI approaches.

Additionally, a steady-state               

Furthermore, a comparison between the AMI method in OpenFOAM and the sliding mesh method in Ansys-Fluent is conducted using identical meshes. The results of this comparison are presented in Appendix 1.           
\begin{figure}[htbp!]
    \centering
    \begin{subfigure}{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/TaylorCouetteFlow_AllSoftware.png}
        \caption{Comparison of velocity distribution using each method.}
        \label{fig:TaylorCouetteFlow_AllSoftware_Deviation}
    \end{subfigure}
	\\
    \begin{subfigure}{0.8\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures/TaylorCouetteFlow_Performance_AllSoftware.png}
        %\caption{Resolution and computational time comparison for each method.}
        \label{fig:Taylor_CouetteFlow_AllSoftware_TimeTaken}
    \end{subfigure}
    \caption{Results of Taylor-Couette flow analysis using different methods.}
    \label{fig:Taylor_Couette_Flow_All_Software}
\end{figure}
\thispagestyle{empty}
